Rectilinear Steiner Trees in Narrow Strips

A rectilinear Steiner tree for a set $P$ of points in $\mathbb{R}^2$ is a tree that connects the points in $P$ using horizontal and vertical line segments. The goal of Minimal Rectilinear Steiner Tree is to find a rectilinear Steiner tree with minimal total length. We investigate how the complexity of Minimal Rectilinear Steiner Tree for point sets $P$ inside the strip $(-\infty,+\infty)\times [0,\delta]$ depends on the strip width $\delta$. We obtain two main results. 1) We present an algorithm with running time $n^{O(\sqrt{\delta})}$ for sparse point sets, that is, point sets where each $1\times\delta$ rectangle inside the strip contains $O(1)$ points. 2) For random point sets, where the points are chosen randomly inside a rectangle of height $\delta$ and expected width $n$, we present an algorithm that is fixed-parameter tractable with respect to $\delta$ and linear in $n$. It has an expected running time of $2^{O(\delta \sqrt{\delta})} n$.

==> 3_approx.tex <==
\section{An approximation algorithm for sparse point sets}
$$ A_{i} = {i \mid T} $$

In this appendix, we present two lemmas.
The first lemma shows that a minimal \emph{monotonic} rectilinear Steiner tree (MMRST) can be found in $O(n)$ time, assuming the points are given sorted on their $x$-coordinates.
The second lemma shows that a separator can indeed be crossed in $n^{\Theta(\sqrtd)}$ different ways given only the points to its left, thus proving that any algorithm faster than the algorithm provided in Section~\ref{sec:sparse} must be significantly different.

We will first focus on MMRSTs.
\begin{lemma}\label{lem:misc:mmrst}
Let $P$ be a set of $n$ terminals in $\Reals^2$, sorted on their $x$-coordinates.
Then a minimal monotonic rectilinear Steiner tree can be found in $O(n)$ time.
\end{lemma}
\begin{proof}
We note that Observation~\ref{obs:prelim:hanan} also holds for the MMRST problem.
The proof of this is analogous to the proof of the original observation.
Furthermore, we note that any two points who share an $x$-coordinate must be connected by a vertical line segment;
otherwise, the separator directly to their left of to their right must be crossed at least twice.
Therefore, the problem can be reformulated as the problem to find an MMRST on a set of vertical line segments $S_1,...S_m$.
We will now give a greedy algorithm solving this problem.
Specifically, we define
\begin{quotation}
$A[i]$ := a MMRST on $S_1,...,S_i$ with a maximal rightmost complete vertical segment.
\end{quotation}
We will show later that the maximal rightmost complete vertical segment is unique.
For brevity, we will write `rightmost segment' to denote the rightmost complete vertical segment.
We take $A[1] \mydef S_1$.
The recursive function is quite simple:
If the segment $S_{i+1}$ and the rightmost segment of $A[i]$ can be connected with a single horizontal edge, then $A[i+1]$ is the resulting MMRST.
Otherwise, w.l.o.g. let $S_{i+1}$ be below the rightmost segment of $A[i]$.
Then, we add two edges: a horizontal edge from the bottom endpoint of the rightmost segment of $A[i]$ to the right, and a vertical edge from the topmost point of $S_{i+1}$, such that these edges share an endpoint.
The resulting MMRST is $A[i+1]$.
See Figure~\ref{fig:misc:mmrst} for an example.
\begin{figure}
\begin{center}
\includegraphics{figures/misc/mmrst}
\caption{An example of an MMRST found as described in Lemma~\ref{lem:misc:mmrst}.
In red, $A[2]$.}
\label{fig:misc:mmrst}
\end{center}
\end{figure}

The running time of this algorithm is trivial --- recall that the points were given sorted on their $x$-coordinate --- so all that remains is to prove the correctness.
Clearly, $A[1] \mydef S_1$ is the only MMRST;
therefore, the maximal rightmost segment is indeed unique.
Now, suppose $A[i+1]$ is formed by adding a single horizontal edge $e$ and $S_{i+1}$ to $A[i]$.
Since $A[i]$ is an MMRST, so is $A[i+1]$.
We will now show that the rightmost segment is indeed maximal.
Let $T$ be any MMRST on $S_1,...,S_{i+1}$.
Let $T'$ be the part of $T$ to the right of $S_i$, and $e'$ its horizontal edge.
Since $A[i]$ has a maximal rightmost segment, the tree $A[i] \cup T'$ must also be an MMRST.
Since $A[i+1]$ and $T$ are both MMRSTs, we get:
\[\|T'\| = \|T\|-\|A[i]\| = \|A[i+1]\|-\|A[i]\| = |e| + |S_{i+1}| = |e'| + |S_{i+1}|.\]
Since $T'$ contains at least the edge $e'$ and the segment $S_{i+1}$, it consists of exactly these two parts.
Therefore, its rightmost segment is indeed $S_{i+1}$.
The case where $A[i+1]$ is formed by adding two edges and $S_{i+1}$ to $A[i]$ can be proven analogously. 

Since we have now shown that $A[1]$ indeed has the required properties and that if $A[i]$ has these properties, so does $A[i+1]$, we conclude that $A[m]$ contains an MMRST on $S_1,...,S_m$, and therefore an MMRST on $P$.
\end{proof}

\begin{lemma}
Let $\delta > 0$ be fixed.
Let $P$ be a sparse point set with sparseness constant $k$.
Then the MMRST is an $\frac{2+k\delta}{2+\delta}$-approximation of the MRST.
This bound is tight.
\end{lemma}
\begin{proof}
\ha{TODO}
\end{proof}

==> 5_random_old.tex <==
\section{Random point sets inside a narrow rectangle}\label{sec:random}
In this section, we give an algorithm with $\min \{n^{O(\sqrtd)}, 2^{O(\delta \sqrtd)} n\}$ expected running time for random point sets.
Specifically, we assume the points in $P$ are taken independently uniformly at random from the rectangle $[0,n] \times [0, \delta]$.
Our proof has the following five steps, which will be explained in detail later.

\begin{itemize}
\item The spacings $\Delta_i \mydef x_{i+1}-x_i$ play an important role in the analysis of the algorithm.
    It will be convenient to assume that the $\Delta_i$ are independent.
    However, when the $x$-coordinates of the points are generated uniformly at random 
    in the interval $[0,n]$, this is not quite true. In the first step, we therefore describe a method
    to generate a random point set in a rectangle of randomly generated height $\ovd$, 
    and we show how to relate the expected running times in these two settings. 
    \mdb{Say that this is similar to our previous paper.}
\item For our second step, we will give a pattern of points: the \emph{hard wall}.
    While extremely rare, it splits the problem into two 
    completely independent subproblems.
    Our algorithm works by first finding these hard walls, 
    and then using one of two different algorithms on the resulting subproblems.
\item In the third step, we consider the case $\ovd \leq 2$ or $\ovd \geq 2 \delta+2$. 
      In this case, we run the $2^{O(\sqrt{n} \log n)}$ algorithm 
      \mdb{Which one? citation?}
      on our subproblems.
      \mdb{I am still confused about how this actually works. Say that I have generated a point set $P$ by drawing points
      uniformly at random from $[0,n]\times[0,\delta]$. I give this point set to you, and you now have to give me the answer, where the expected time is whatever. What does it mean that $\ovd \leq 2$ or $\ovd \geq 2 \delta+2$? Probably we should run all algorithms in parallel and stop when the first one is done?
      What does it mean to check the condition for being a hard wall wrt $\ovd$? Should we just check it for $\delta?$}
\item For the fourth step, we will give another pattern of points, which we call a \emph{soft wall}.
    It is extremely common when $2 < \ovd$, even under limiting assumptions, 
    and pinpoints a separator which is crossed $O(\sqrtd)$ times.
\item In the fifth step, we consider the case $2 < \ovd < 2 \delta+2$. 
    In this case, we run a variant of the $n^{O(\sqrtd)}$ sparse point set algorithm on our subproblems, 
    using only the separators given by the soft walls.
\end{itemize}
\ha{insert samenvatting werking algo, in de vorm van pseudocode}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\mypara{Step 1: Another way of generating points, with independent $\Delta_i$.}
    \mdb{This text should not be copy-paste from the previous paper.
    (I did not check if it is :)}
    \ha{voor alle niet-direct-noodzakelijke onderdelen verwijzen naar vorige paper}
Let us first extend the definition of spacings with $\Delta_0 = x_1$, and $\Delta_n = n - x_n$.
Note that $\sum_{i=0}^n \Delta_i = n$.
As $n$ goes to infinity, the $\Delta_i$ become more and more independent.
True independence would greatly simplify the calculation of the running time.
Therefore, let us take a look at a different way of generating our point set.

First, we generate $n+1$ independent exponentially distributed variables, $\Delta_0,...,\Delta_n \sim \Exp (1)$.
Using these, we compute the $x$-coordinates of our points, defined as $x_i := \sum_{j=0}^{i-1} \Delta_i$ for $1 \leq i \leq n$;
note that $\Delta_n$ is not yet used.
Define $\ovd := \delta \, (\sum_{i=0}^n \Delta_i)/n$.
Note that $\ovd$ will very likely be relatively close to $\delta$, since $\sum_{i=0}^n \Delta_i$ converges to a normal distribution with mean $n+1$ and variance $\sqrt{n+1}$ when $n \rightarrow \infty$.
Finally, we generate the other coordinates 
    by picking $n$ independent uniformly distributed points in $[0,\ovd]$. \mdb{You mean the $y$-coordinates? Then write:
    Finally, we generate the $y$-coordinates of the point by
    picking each $y_i$ uniformly and independently from the
    interval~$[0,\ovd]$}
Combining these gives us $n$ points in the rectangle $[0, n \, \ovd / \delta] \times [0,\ovd]$.

A point set generated this way has two important properties.
First of all, the $\Delta_i$ are now independent.
Second, when the coordinates of the points are re-scaled with a factor $\delta / \ovd$, the points have a distribution equal to the distribution of a point set generated by taking $n$ uniform points in the rectangle $[0,n] \times [0,\delta]$ \cite{daley2007introduction}.
Therefore, the expected running time of an algorithm on a point set generated this way is equal to the expected running time of an algorithm on a point set generated in the normal way.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\mypara{Step 2: The hard wall.}
In this step, we will show a pattern of points which allows the problem to be split into two independent subproblems.
Recall that $P[i,j] \mydef \{p_i,...,p_j\}$.
We define a \emph{hard wall} to be a set of five points $P[i,i+4]$ such that (i) $\Delta_i,...,\Delta_{i+3} > \ovd$ and (ii) $y_{i+1} < y_{i+2} < y_{i+3}$.
See Figure~\ref{fig:random:hardwall} for an example of a hard wall.
\begin{figure}
\begin{center}
\includegraphics{figures/random/hardwall}
\caption{An example of a hard wall}
\label{fig:random:hardwall}
\end{center}
\end{figure}
\begin{lemma}\label{obs:random:hardwall}
Let $P[i,i+4]$ be a hard wall.
Let $T_1$ be an MRST on $P[1,i+2]$ and let $T_2$ be an MRST on $P[i+2,n]$.
Then $T_1 \cup T_2$ is an MRST on $P$.
\mdb{Do we need: then $\|T\| = \|T_1\| + \|T_2\|$ and so $T_1 \cup T_2$ is an MRST on $P$.}
\end{lemma}
\begin{proof}
\mdb{Is the following shorter proof also convincing?
Let $T$ be a Hwang tree on~$P$.
By Observation~\ref{obs:gen:paralleledges} we know that an MRST on $P$
is monotonic at $s_i,...,s_{i+3}$. The monotonicity at $s_{i+1}$ and $s_{i+2}$
implies that $\degr_T(p_{i+2})$, the degree of $p_{i+2}$ in $T$, is at most~2. 
If $\degr_T(p_{i+2})=2$ then splitting $T$ at $p_{i+2}$ results
in subtrees on $P[1,i+2]$ and $P[i+2,n]$---this follows from the
monotonicity at $s_{i+1}$ and $s_{i+2}$---and so we are done. 
Now assume for a contradiction that $\degr_T(p_{i+2})=2$. Then the incident edge
if $p_{i+2}$ must be vertical. Assume without loss of generality that $p_{i+2}$
is the top endpoint of this edge. But then the (single) edge of $T$ crossing $s_{i+2}$ must reach the vertical
line through $p_{i+3}$ at a point $q$ that lies somewhere below~$p_{i+3}$. The
monotonicity at $s_{i+3}$ then implies that $q$ must be connected
tp $p_{i+3}$ by a vertical segment, thus creating a U-shape and contradicting that $T$ is a Hwang tree.
}
From Observation~\ref{obs:gen:paralleledges} we directly get that any MRST is monotonic at $s_i,...,s_{i+3}$. \mdb{Hmm, Obs 3 is formulated slightly differently.}
Therefore, an MRST $T$ on $P$ of which the edges crossing $s_{i+1}$ and $s_{i+2}$ are in different full components (if such an MRST exists) has the same total length as $T_1 \cup T_2$.
Let $T$ be a Hwang tree on $P$.
We will now show that $T$ crosses $s_{i+1}$ at a height between $y_{i+1}$ and $y_{i+2}$ (inclusive).
By symmetry, we can then conclude that $T$ must cross $s_{i+2}$ at a height between $y_{i+2}$ and $y_{i+3}$, thereby proving that the two edges of $T$ crossing $s_{i+1}$ and $s_{i+2}$ are in different full components.

First, recall that since $T$ is a Hwang tree, it does not contain a `U' formed by an edge between two segments with a terminal on the same side.
See Figure~\ref{fig:prelims:hwangtrees} for an example.
Furthermore, note that since $T$ is monotonic at $s_i$ and at $s_{i+1}$, the edge crossing $s_{i+1}$ must be incident to a segment which has $p_{i+1}$ as an endpoint.
Analogously, since $T$ is monotonic at $s_{i+1}$ and $s_{i+2}$, the edge crossing $s_{i+1}$ must be incident to a segment which has $p_{i+2}$ as an endpoint.
Combining these three observations, we conclude that the edge crossing $s_{i+1}$ has a height between $y_{i+1}$ and $y_{i+2}$ (inclusive).

In conclusion, since the edge of $T$ crossing $s_{i+1}$ is lower than $p_{i+2}$, while the edge of $T$ crossing $s_{i+2}$ is higher than $p_{i+2}$, they must be in different full components.
Therefore, $T$ has the same length as $T_1 \cup T_2$, proving the statement.
\end{proof}
Since the $\Delta_j$ are independent and exponentially distributed, the probability that $P[i,i+4]$ is a hard wall is $e^{-4 \ovd} / 6$ for all $i$.

Our algorithm starts by splitting the problem using these hard walls. To this end
we first check for each $i=5j+1$ with $j\in\{0,\ldots,\floor{n/5}-1\}$, in $O(n)$ time whether $P[i,i+4]$ forms a hard wall.
Note that the corresponding probabilities are independent.
Then, we run one of two algorithms on the resulting subproblems, as will be explained in the remaining steps.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\mypara{Step 3: The case $\ovd \leq 2$ or $\ovd \geq 2 \delta + 2$.}
If $\ovd \leq 2$ or $\ovd \geq 2 \delta + 2$, we run the $2^{O(\sqrt{n} \log n)}$ algorithm on the resulting subproblems. \mdb{citation}
We will now show that this case takes only $O(n)$ expected time.

We will start with the subcase $\ovd \leq 2$.
    \mdb{Hmm, at various places we are using that the $\Delta_i$ are independent. However, here we are in the case $\delta^*\leq 2$. Do we still know that the $\Delta_i$ are independent \emph{conditioned to the event $\delta^*\leq 2$?}}
In this subcase, each of the subproblems contains $5\;\text{Geom}(e^{-4 \ovd} / 6)$ points, 
\mdb{Say what Geom is, and explain why you get this bound.}
with the exception that it is capped at the remaining number of points.
\mdb{Do you mean: except possible the last subproblem, since the distribution is capped at $n$. Or something like that?}
Since we run a subexponential algorithm on these subproblems and $\ovd\leq 2$, we have a $O(1)$ expected running time per subproblem.
\mdb{Explain in one line?}

For the subcase $\ovd \geq 2 \delta + 2$, we will use the Chernoff bound to show that the probability of this case occurring is extremely small.
    \mdb{This is the same as in the other paper, right? Then we could just cite that. Do we already have an arxiv version that contains this?}
\begin{align*}
\PP\left[\ovd > 2 \delta + 2\right] &= \PP\left[\delta\br{\sum_{i=0}^n \Delta_i}/n > 2 \delta + 2\right] \\
	&= \PP\left[\sum_{i=0}^n \Delta_i > 2 n (1+1/\delta)\right] \\
	&\leq \min_{t > 0} e^{-2 t n (1+1/\delta)} (\EE[e^{t \Delta_1}])^{n+1}
		& \text{by the Chernoff bound}\\
	&\leq e^{- n (1+1/\delta)} (\EE[e^{\Delta_1/2}])^{n+1}
		& \text{$t = 1/2$} \\
	&= e^{- n (1+1/\delta)} \br{\int_{x=0}^{\infty} e^{x/2} e^{-x} \diff x }^{n+1}
		& \Delta_1 \sim \Exp(1) \\
	&= e^{- n (1+1/\delta)} 2^{n+1} \\
	&< 2 e^{-n/4},
\end{align*}
which is exponentially decreasing in $n$.
The total expected time needed for this case is therefore bounded by $2^{-n/4} \cdot 2^{O(\sqrt{n} \log n)} = O(1)$ per subproblem.

Since both subcases need $O(1)$ expected time per subproblem, the case $\ovd \leq 2$ or $\ovd \geq 2 \delta + 2$ takes $O(n)$ expected time in total.
From now on, we will consider the case $2 < \ovd < 2 \delta + 2$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\mypara{Step 4: The soft wall.}
    \mdb{PArhaps better to put this as a part of step 5?}
We define a \emph{soft wall} to be a set of $\cisqrtod+1$ points $P[i,i+\cisqrtod]$ with the property $x_{i+\cisqrtod} - x_i > \sqrtod/4$.
See Figure~\ref{fig:random:softwall} for an example of a soft wall.
\begin{figure}
\begin{center}
\includegraphics{figures/random/softwall}
\caption{An example of a soft wall}
\label{fig:random:softwall}
\end{center}
\end{figure}
Now, Lemma~\ref{lem:gen:sqrtdeltacrossings} directly gives us that $s_i$ is crossed at most $O(1+\sqrtod)=O(\sqrtod)$ times.
We want to calculate a lower bound on the probability that $P[i,i+\cisqrtod]$ is a soft wall.
However, we will be searching for these soft walls in each of the subproblems created by the hard walls.
Therefore, we assume that no $\Delta_j$ is larger than $\ovd$.
We get:
\begin{align*}
& \PP \left[x_{i+\csqrtod} - x_i > \sqrtod/4\right] \\
&= 1 - \PP \left[\sum_{j=i}^{i+\csqrtod-1} \Delta_j \leq \sqrtod/4 \right]\\
&\geq 1 - \min_{t>0} e^{t \sqrtod/4} \br{ \EE[e^{-t\Delta_1}]}^{\csqrtod-1}
&\text{by the Chernoff bound}\\
&\geq 1 - \min_{t>0} e^{t \sqrtod /4} \br{ \int_{x=0}^{\ovd} e^{-tx}e^{-x} \frac{1}{1-e^{-\ovd}} }^{\csqrtod-1}
&\Delta_1 \sim \Exp(1) \text{ and } \Delta_1 \leq \ovd\\
&= 1 - \min_{t>0} e^{t \sqrtod/4} \br{\frac{e^{\ovd }-e^{-\ovd t}}{\br{e^{\ovd }-1} (t+1)}}^{\csqrtod-1}\\
&> 1 - \min_{t>0} 2e^{t \sqrtod/4} \br{\frac{1}{t+1}}^{\sqrtod-1}\\
&= 1 - 2e^{3\sqrtod/4 -1} \br{\frac{1}{4 -4/\sqrtod}}^{\sqrtod-1}
&t = 3 -4/\sqrtod\\
&> 1 - 2^{3 - 3\sqrtod}
\end{align*}
This finishes the explanation of the soft wall.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\mypara{Step 5: The case $2 < \ovd < 2 \delta + 2$.}
We are now ready to create the algorithm we run on the subproblems in the case $2 < \ovd < 2 \delta + 2$.
We start by searching for soft walls.
Specifically, we check whether $(p_i,...,p_{i+\cisqrtod})$ forms a wall for every $i$ divisible by $\cisqrtod$.
Note that the corresponding probabilities are independent.
We then run the sparse point set algorithm as usual, but using only the separators pinpointed by the soft walls.
Furthermore, instead of brute-forcing every subsubproblem between two separators, we run the $2^{O(\sqrt{n}\log n)}$ algorithm.
    \mdb{Which one?}
Let us define $m$ as the number of points in our subproblem.
Note that we fewer than $m$ subsubproblems in total, each containing at most $(\text{Geom}(1 - 2^{3 - 3\sqrtod})+1)\cisqrtod+1$ points.
The total expected time needed per subsubproblem therefore is
\begin{align*}
    &\sum_{i=1}^\infty 2^{\sqrt{i \csqrtod +1}\log \br{i \csqrtod+1}} \br{2^{3-3\sqrtod}}^{i-1} \br{1 - 2^{3-3\sqrtod}}\\
    &< \; 2^{3 \sqrtod} \sum_{i=1}^\infty 2^{\sqrt{3 i\sqrtod}\log \br{3 i \sqrtod}} \cdot 2^{-i \sqrtod/2} 
    & \text{since } \ovd > 2\\
    &< \; 2^{3 \sqrtod} \sum_{i=1}^\infty 2^{\sqrtod  (6 i^{3/4} - i / 2)} \\
    &= \; 2^{3\sqrtod} \br{ \sum_{i=1}^{331775} 2^{\sqrtod  (6 i^{3/4} - i / 2)} + \sum_{i=331776}^\infty 2^{\sqrtod  (6 i^{3/4} - i / 2)}} \\
    &< \; 2^{3\sqrtod} \br{ 331775 \cdot 2^{2187 \sqrtod /2} + \sum_{i=331776}^\infty 2^{- i / 4}} \\
    &= \; 2^{O\br{\sqrtod}}
\end{align*}
Analogously to the original spare point set algorithm, there are $m^{O(\sqrtod)}$ possible crossing patterns per separator.
In total, this algorithm therefore takes $m \, \cdot m^{O(\sqrtod)} \cdot 2^{O\br{\sqrtod}} = m^{O(\sqrtd)}$ expected time.

Now, all that remains is calculating the expected running time of our main random point set algorithm in this case.
Clearly, it runs in at most expected $n^{O(\sqrtd)}$ time, since splitting up the problem using the hard walls can only speed up the algorithm.

Let $\labda, \mu \geq 1$ be such that the $m^{O(\sqrtd)}$ expected running time algorithm runs in $m^{\labda \sqrtd}$ expected time, and that the probability of a hard wall is $2^{- \mu \delta}$.
Let $X$ be the distribution of the number of points of a subproblem.
Then the total expected time needed per subproblem is:
$$ 
\EE[X^{\labda \sqrtd}]
\leq \sum_{k=0}^\infty \br{5k+6}^{\labda \sqrtd} 2^{-\mu \delta} (1-2^{-\mu \delta})^{k} < O(1) + 2^{-\mu \delta} \sum_{k=2}^\infty 2^{4\labda \sqrtd \log k -2^{-\mu \delta} k} $$
We split the sum into two parts, with $M=64 \labda^2 \delta 2^{2 \mu \delta}$. We get
\begin{align*}
&2^{-\mu \delta} \sum_{k=2}^\infty 2^{4\labda \sqrtd \log k -2^{-\mu \delta} k}\\
&< 2^{-\mu \delta} \br{ \sum_{k=2}^{M-1} 2^{4\labda \sqrtd \log k -2^{-\mu \delta} k} +  \sum_{k=M}^\infty 2^{-2^{-\mu \delta} k/2} }\\
&< 2^{-\mu \delta} M 2^{\max_{k} \br{\labda \sqrtd \log k -2^{-\mu \delta} k}} + \frac{2^{-\mu \delta}}{1-2^{-2^{-\mu \delta-1}}} \\
&= 2^{-\mu \delta} M 2^{\labda \sqrtd \log (\labda \sqrtd 2^{\mu \delta} \ln 2) -2^{-\mu \delta} (\labda \sqrtd 2^{\mu \delta} \ln 2)} + O(1) \\
&= 2^{O(\delta \sqrtd)}, \\
\end{align*}
\ha{toevoegen dat breuk convergeert naar 2/log2}
bringing the total expected running time to $O(n) \cdot (O(1) + 2^{O(\delta \sqrtd)}) = 2^{O(\delta \sqrtd)} n$.

In conclusion, our main random point set algorithm uses $O(n)$ expected running time for the case $\ovd \leq 2$ or $\ovd \geq 2 \delta + 2$, and it uses $\min\{n^{O(\sqrtd)},2^{O(\delta \sqrtd)} n\}$ for the case $2 < \ovd < 2 \delta + 2$.
Therefore:
\begin{theorem}
Let $P$ be a point set of $n$ points taken uniformly at random from the rectangle $[0,n] \times [0,\delta]$.
Then an MRST on $P$ can be found in $\min\{n^{O(\sqrtd)},2^{O(\delta \sqrtd)} n\}$ expected time.
\end{theorem}

==> geomsep.tex <==
\section{Geometric separators - full proofs and definitions}
First, some definitions. Let $P$ be a set of \emph{sites} in ${\mathbb{R}^+}^d$. We will only consider MRSTs on the Hanan grid, such that no flips or slides are possible towards the origin. Let $T$ be a Minimal Rectilinear Steiner Tree (MRST) on $P$. As with all graphs, $T$ has \emph{vertices} and \emph{edges} between these vertices. The vertices of $T$ can be split into three kinds: the $n$ \emph{sites}, the \emph{Steiner points}, which are the non-sites with degree at least 3, and the \emph{corners}. The set of vertices is defined in such a way that $T$ has no vertices of degree 2 of which the edges go in opposite directions. We define a \emph{superedge} to be a path from a non-corner to a non-corner through corners.

We will start with some observations:

\begin{observation}
Let $T$ be a MRST. Then $T$ is a tree.
\end{observation}
\begin{proof}
Trivial.
\end{proof}

\begin{observation}
Let $T$ be a MRST. Then each vertex of $T$ has degree $\leq 2d$.
\end{observation}
\begin{proof}
Trivial, because rectilinear.
\end{proof}

\begin{observation}
Let $T$ be a MRST. Then $T$ has at most $n-1$ Steiner points.
\end{observation}
\begin{proof}
Trivial, because tree.
\end{proof}

\begin{observation}
Let $T$ be a MRST. Then $T$ has $< 2dn$ edges.
\end{observation}
\begin{proof}
Note that all superedges contain $\leq d$ edges. Note that there are (no. of Steiner points + no. of sites - 1) superedges, because tree. Therefore, the total number of edges is at most
$$(\text{no. of Steiner points} + \text{no. of sites} - 1)d \leq (n-1+n-1)d < 2dn.$$
\end{proof}

Since we'll check stuff from the top down, we now introduce but don't prove the following lemma:
\begin{lemma} \label{lem:box}
Let $n > d$. Let $T$ be a MRST with $e$ edges. Then there exists a $d$-box such that (i) at most $2n/3$ of the sites are inside it, (ii) at most $2n/3$ of the site are outside it, and (iii) at most $O(d^2 e^{1-1/d})$ of the edges cross the box boundary.
\end{lemma}
Note that since $e < 2dn$, we have $O(d^{3-1/d} n^{1-1/d})$ edges crossing the box boundary.
\begin{observation} \label{obs:boxnr}
There is a set of $n^{O(d)}$ candidate boxes for Lemma \ref{lem:box}.
\end{observation}
\begin{proof}
Since all vertices are on the Hanan grid, there are only at most $\binom{n+1}{2}^d = n^{O(d)}$ possible boxes.
\end{proof}
Using the above two lemmas, we get the following theorem.
\begin{theorem}
MRST can be solved in $2^{d^{O(d)}} n^{O(d^3 n^{1-1/d})}$ time.
\end{theorem}
\begin{proof}
The algorithm is as follows:
\begin{itemize}
\item Guess the box of Lemma~\ref{lem:box} out of the $n^{O(d)}$ candidates (see Observation \ref{obs:boxnr}).
\item Guess the $\leq O(d^{3-1/d} n^{1-1/d})$ points where edges cross the box boundary.
\item Guess how these points are connected on the inside, and how they are connected on the outside.
\item Solve the remaining problems recursively.
\item When at most $d^{c_1 d}$ points remain, brute-force the solution.
\end{itemize}
The running time then satisfies:
$$T(n) \leq BFT + NOIHGAB^{O(d^{3-1/d} n^{1-1/d})} PC (T(2n/3) + T(n/3))$$
with base case $T(d^{O(d)}) = BF$,
where $BFT$ is the BoxFinderTime, $NOIHGAB$ is NumberOfIntersectionsHananGridAndBox, $PC$ is PossibleConnections, and $BF$ is BruteForce.

%----------------------------------------
% aantekeningen
%----------------------------------------

The paper claims:
- $BFT$ is small enough.
- $NOTHGAB$ is $< 2dn^{d-1}$.
- The boundary is crossed at $O(d^2 n^{1-1/d})$ places.
- For $C$ crossing points, there are $< 4^C C!$ possible connections.
- Brute force takes $2^{O(n)}$ time.
- Total is $$n^{O(d)} (8dn^{d-1})^{d^2 n^{1-1/d}}$$

$T(n) \leq BFT + NOIHGAB^{O(d^{3-1/d} n^{1-1/d})} PC (T(2n/3) + T(n/3))$
$T(n) \leq (2dn^{d-1})^{O(d^2 n^{1-1/d})} 4^{O(d^2 n^{1-1/d})} (O(d^2 n^{1-1/d}))! (T(2n/3) + T(n/3))$
$T(n) \leq (8dn^{d-1})^{O(d^2 n^{1-1/d})} (O(d^2 n^{1-1/d}))! (T(2n/3) + T(n/3))$
$$T(n) \leq (8dn^{d-1})^{O(d^2 n^{1-1/d})} (T(2n/3) + T(n/3))$$

Conclusie:
Waarschijnlijk denkt paper dat $BFT = n^{O(d)}$, en gebruiken ze $BFT *$ ipv $BFT +$. Verder is een $O()$ vergeten in de exponent, of stond hij er eerder te veel (wsl eerste).

%----------------------------------------
% eind aantekeningen
%----------------------------------------
Assumption:
$$T(n) \leq n^{O(d)} (8dn^{d-1})^{O(d^2 n^{1-1/d})} (T(2n/3) + T(n/3))$$
$$T(n) \leq n^{O(d)} (dn^{d-1})^{O(d^2 n^{1-1/d})} (T(2n/3) + T(n/3))$$
$$T(n) \leq n^{c_3 d} (dn^{d-1})^{c_4 d^2 n^{1-1/d}} (T(2n/3) + T(n/3))$$
\textbf{Claim:} $T(n) = 2^{d^{O(d)}} n^{O(d^3 n^{1-1/d})}$.\\
\textbf{Claim:} $T(n) = 2^{d^{c_1 d}} n^{c_2 d^3 n^{1-1/d}}$.\\
\textbf{Base case:} $T(d^{O(d)}) = 2^{d^{O(d)}} d^{d^{O(d)}}$: is ok for $c_1$ large enough.\\
\textbf{Induction:} To prove: for all $c_3, c_4$ there exist $c_1, c_2$ such that $T(3n) \geq (3n)^{c_3 d} (d(3n)^{d-1})^{c_4 d^2 (3n)^{1-1/d}} (T(2n) + T(n))$
$$2^{d^{c_1 d}} (3n)^{c_2 d^3 (3n)^{1-1/d}} \geq (3n)^{c_3 d} (d(3n)^{d-1})^{c_4 d^2 (3n)^{1-1/d}} \br{2^{d^{c_1 d}} (2n)^{c_2 d^3 (2n)^{1-1/d}} + 2^{d^{c_1 d}} n^{c_2 d^3 n^{1-1/d}}}$$
$$(3n)^{c_2 d^3 (3n)^{1-1/d}} \geq (3n)^{c_3 d} (d(3n)^{d-1})^{c_4 d^2 (3n)^{1-1/d}} \br{(2n)^{c_2 d^3 (2n)^{1-1/d}} + n^{c_2 d^3 n^{1-1/d}}}$$
$$(3n)^{c_2 d^3 (3n)^{1-1/d}-c_3 d} \geq d^{c_4 d^2 (3n)^{1-1/d}} (3n)^{(d-1) c_4 d^2 (3n)^{1-1/d}} \br{(2n)^{c_2 d^3 (2n)^{1-1/d}} + n^{c_2 d^3 n^{1-1/d}}}$$
$$(3n)^{(d c_2-(d-1) c_4) d^2 (3n)^{1-1/d}-c_3 d} \geq d^{c_4 d^2 (3n)^{1-1/d}} \br{(2n)^{c_2 d^3 (2n)^{1-1/d}} + n^{c_2 d^3 n^{1-1/d}}}$$
Sufficient:
$$(3n)^{(d c_2-(d-1) c_4) d^2 (3n)^{1-1/d}-c_3 d} \geq 2 d^{c_4 d^2 (3n)^{1-1/d}} (2n)^{c_2 d^3 (2n)^{1-1/d}}$$
Sufficient:
$$(3n)^{(d 10(c_4+c_3)-d c_4) d^2 (3n)^{1-1/d}-c_3 d} \geq 2 d^{c_4 d^2 (3n)^{1-1/d}} (2n)^{10(c_4+c_3) d^3 (2n)^{1-1/d}}$$
Sufficient:
$$(3n)^{9(c_4+c_3) d^3 (3n)^{1-1/d}} \geq 2 d^{c_4 d^2 (3n)^{1-1/d}} (2n)^{10(c_4+c_3) d^3 (2n)^{1-1/d}}$$
$$2^{log_2(3) 9(c_4+c_3) d^3 (3n)^{1-1/d} - 1 - 10(c_4+c_3) d^3 (2n)^{1-1/d}} n^{9(c_4+c_3) d^3 (3n)^{1-1/d}-c_4 d^2 (3n)^{1-1/d}-10(c_4+c_3) d^3 (2n)^{1-1/d}} \geq 1$$
$$2^{24 (c_4+c_3) d^3 n^{1-1/d} - 1 - 20(c_4+c_3) d^3 n^{1-1/d}} n^{9(c_4+c_3) d^3 (3n)^{1-1/d}-c_4 d^2 (3n)^{1-1/d}-10(c_4+c_3) d^3 (2n)^{1-1/d}} \geq 1$$
$$2^{3 (c_4+c_3) d^3 n^{1-1/d}} n^{9(c_4+c_3) d^3 (3n)^{1-1/d}-c_4 d^2 (3n)^{1-1/d}-10(c_4+c_3) d^3 (2n)^{1-1/d}} \geq 1$$
$$n^{9(c_4+c_3) d^3 (3n)^{1-1/d}-c_4 d^2 (3n)^{1-1/d}-10(c_4+c_3) d^3 (2n)^{1-1/d}} \geq 1$$
$$9(c_4+c_3) d^3 (3n)^{1-1/d}-c_4 d^2 (3n)^{1-1/d}-10(c_4+c_3) d^3 (2n)^{1-1/d} \geq 0$$
$$9 d^3 (3n)^{1-1/d}-d^2 (3n)^{1-1/d}-10 d^3 (2n)^{1-1/d} \geq 0$$
$$9 d 3^{1-1/d}- 3^{1-1/d}-10 d 2^{1-1/d} \geq 0$$
$$(9 d-1) 3^{1-1/d}-10 d 2^{1-1/d} \geq 0$$
$$(9 d-1)\sqrt{3} -10 \sqrt{2}  d \geq 0$$
$$17\sqrt{3} -20 \sqrt{2} \geq 0$$
Check!




\end{proof}
